Learning Models over Relational Data using Sparse Tensors and Functional Dependencies

Integrated solutions for analytics over relational databases are of great practical importance as they avoid the costly repeated loop data scientists have to deal with on a daily basis: select features from data residing in relational databases using feature extraction queries involving joins, projections, and aggregations; export the training dataset defined by such queries; convert this dataset into the format of an external learning tool; and train the desired model using this tool. These integrated solutions are also a fertile ground of theoretically fundamental and challenging problems at the intersection of relational and statistical data models. This article introduces a unified framework for training and evaluating a class of statistical learning models over relational databases. This class includes ridge linear regression, polynomial regression, factorization machines, and principal component analysis. We show that, by synergizing key tools from database theory such as schema information, query structure, functional dependencies, recent advances in query evaluation algorithms, and from linear algebra such as tensor and matrix operations, one can formulate relational analytics problems and design efficient (query and data) structure-aware algorithms to solve them. This theoretical development informed the design and implementation of the AC/DC system for structure-aware learning. We benchmark the performance of AC/DC against R, MADlib, libFM, and TensorFlow. For typical retail forecasting and advertisement planning applications, AC/DC can learn polynomial regression models and factorization machines with at least the same accuracy as its competitors and up to three orders of magnitude faster than its competitors whenever they do not run out of memory, exceed 24-hour timeout, or encounter internal design limitations.

==> gradient.tex <==
\section{The inner loop of BGD}
%Computing the parameters of the optimization problem}
\label{sec:gradient}

\mjs{Merge this in with the previous Section}

As shown in Section~\ref{sec:gradientcomputation}, the gradient descent solver repeatedly
computes $J(\vec\theta)$ and $\grad J(\vec\theta)$, which require matrix-vector
and vector-vector multiplications over the quantities
($\vec\Sigma,\vec c, s_Y$). We discuss here the computation that involves the
$\vec\Sigma$ matrix.

It is possible that several entries $\sigma_{ij} \in \vec\Sigma$ map to the same
aggregate query that is computed by AC/DC. Consider, for instance, the following
scalar entries in the feature mapping vector $h$: $h_i(\mv x) = x_a$,
$h_j(\mv x) = x_b\cdot x_c$, $h_k(\mv x) = x_b$, $h_l(\mv x) = x_a\cdot x_c$,
$h_m(\mv x) = x_c$, and $h_n(\mv x) = x_a\cdot x_b$. By definition of
$\vec\Sigma$, any pair-wise product of these entries in $h$ corresponds to one
entry in $\vec\Sigma$. The entries $\sigma_{ij}$, $\sigma_{lk}$, and
$\sigma_{mn}$ (as well as their symmetric counterparts) all map to the same
aggregate
$\SUM(A\cdot B\cdot C)=\sum_{(\mv x, y) \in Q(D)} x_a\cdot x_b \cdot x_c$.  To
avoid this redundancy, we use a sparse representation of $\vec\Sigma$, which
assigns to each distinct aggregate query a list of index pairs $(i,j)$ that
contains one pair for each entry $\sigma_{ij} \in \vec\Sigma$ that maps to this
query.

AC/DC operates directly over the sparse representation of $\vec\Sigma$. Consider
the matrix vector product $\mv p = \vec\Sigma g(\vec\theta)$, and let $A$ be the
root of the variable order $\Delta$. We compute $\mv p$ by iterating over all
aggregate maps $\alpha \in \aggs_{A}$, and for each index pair $(i,j)$ in $\vec\Sigma$ that is
assigned to $\alpha$, we add to the $i$'s entry in $\mv p$ with the product of
$\alpha$ and $j$'s entry in $g(\vec\theta)$. If $i \neq j$, we also add to $j$'s
entry in $\mv p$ with the product of $\alpha$ and $i$'s entry
in $g(\vec\theta)$.

{\bf Regularizer under FDs.}  Section~\ref{SEC:FDS} explains how to rewrite
the regularizer for a ridge linear regression model under the FD
$\mathsf{city} \rightarrow \mathsf{country}$. First, we need to construct the
relation $\mv R(\mathsf{country},\mathsf{city})$, and then compute the inverse
of the matrix $\mv D = (\mv I_{\mathsf{city}} + \mv R^\top \mv R)$. Note that each 
entry $(i,j)$ in $\mv R^\top \mv R$ is $1$, if two cities $\mathsf{city}_i$ and
$\mathsf{city}_j$ are in the same $\mathsf{country}$. Otherwise, the entry
$(i,j)$ is zero.

To facilitate the construction of the matrix $\mv D$, we construct $\mv R$ as a
map that groups the tuples of $\mv R$ by \textsf{country}. Thus, we construct a
mapping from \textsf{country} to the set of cities in this country that occur in
the dataset, which can be computed during the computation of the factorized
aggregates over the variable order.

% When the algorithm finds a particular \textsf{country} $c$, we add all cities
% that are in this country to the payload of the tuple in the map that has $b$ as
% key.
We then use this representation of $\mv R$ to iterate over the payload set, and
for any two cities $\mathsf{city}_i, \mathsf{city}_j$ in the payload set, we
increment the corresponding index $(i,j)$ in $\mv D$ by one. We store $\mv D$
as a sparse matrix in the format used by the Eigen linear algebra library, 
and then use Eigen's Sparse Cholesky Decomposition to compute the inverse of
$\mv D$ and ultimately the solution for the regularizer.


==> high-level-diagram.tex <==
\begin{figure}[ht!]
\centering{
\begin{tikzpicture}[scale=.8, every node/.style={transform shape}]
   \node[data, scale=.8] (FEQ) {feature\\extraction\\ query};
   
   \begin{scope}[shift={($(FEQ)+(3,0)$)}, scale=1, every node/.style={transform shape}]
      \node[inner sep=.3cm, scale=2] at (0,0) (DB) {DB};
      \drawcylinder{1.75}{1.25}{.25}{black}
   \end{scope}
   
   \begin{scope}[shift={($(DB)+(4,0)$)}, scale=1, every node/.style={transform shape}]
      \node[inner sep=.9cm] (0,0) (output_table){};
      \drawtable{1.5}{2}{4}{8}{clr_outofDB}
      \node[clr_outofDB, align=center, scale=.8] at (0,1.4) {materialized\\output};
   \end{scope}
   
   \node[processor, clr_outofDB] at($(output_table)+(3.5,0)$) (ML) {ML tool};
   
   \node[data] at($(ML)+(3,0)$) (theta_opt) {$\vec\theta^*$};
   
   \node[data] at($(ML)+(0,-3)$) (model) {model};
   
   \node[processor, clr_inDB, scale=.8] at($(model)+(-3.5,0)$) (model_reform) {model\\ reformulation};
   
   \node[processor, clr_inDB] at($(DB)+(0, -3)$) (FAQ) {Factorization};
   
   \node[data, clr_inDB] at($(FAQ)+(0, -2.5)$) (sigma_c) {$\vec\Sigma, \vec c$};
   
   \node[processor, clr_inDB, scale=.8] at($(sigma_c)+(4, 0)$) (GD) {Gradient-descent\\Trainer\\\vspace{.2cm}};
   \begin{scope}[shift={($(GD)+(0,-.45)$)}, scale=.3, every node/.style={transform shape}]
      \draw[clr_inDB,->,thick] (-1,.1) arc (170:10:1);
      \draw[clr_inDB,->,thick] (1,-.1) arc (-10:-170:1);
   \end{scope}
   
   \draw[path, clr_outofDB] (FEQ)--(DB);
   \draw[path, clr_outofDB] (DB)--(output_table);
   \draw[path, clr_outofDB] (output_table)--(ML);
   \draw[path, clr_outofDB] (ML)--(theta_opt);
   \draw[path, clr_outofDB] (model)--(ML);
   
   \draw[path, clr_inDB, thick] (model)--(model_reform);
   \draw[path, clr_inDB, thick] (model_reform)--(FAQ) node [midway, above]{$h$};
   \draw[path, clr_inDB, thick] (DB)--(FAQ);
   \draw[path, clr_inDB, thick] (FEQ)--(FAQ);
   \draw[path, clr_inDB, thick] (FAQ)--(sigma_c);
   \draw[path, clr_inDB, thick] (sigma_c)--(GD);
   \draw[path, clr_inDB, thick] (model_reform)--(GD) node [midway, right]{$g$};
   \draw[path, clr_inDB, thick] (GD) -| (theta_opt);
\end{tikzpicture}
}
\caption{{\color{clr_inDB}\bf In-database} vs. {\color{clr_outofDB}Out-of-database} learning: High-level diagram. (See Section~\ref{sec:high-level-diagram}.)}
\label{fig:high-level-diagram}
\end{figure}

